How to Dissect a Muppet: The Structure of Transformer Embedding Spaces

Pretrained embeddings based on the Transformer architecture have taken the NLP community by storm. We show that they can mathematically be reframed as a sum of vector factors and showcase how to use this reframing to study the impact of each component. We provide evidence that multi-head attentions and feed-forwards are not equally useful in all downstream applications, as well as a quantitative overview of the effects of finetuning on the overall embedding space. This approach allows us to draw connections to a wide range of previous studies, from vector space anisotropy to attention weights.

==> shading-gradations/BrownBleen.tex <==
\newcommand{\gradA}{\cellcolor[HTML]{003c30}\color{white}}
\newcommand{\gradB}{\cellcolor[HTML]{295449}\color{white}}
\newcommand{\gradC}{\cellcolor[HTML]{496d63}\color{white}}
\newcommand{\gradD}{\cellcolor[HTML]{6a877e}}
\newcommand{\gradE}{\cellcolor[HTML]{8ba19a}}
\newcommand{\gradF}{\cellcolor[HTML]{adbcb8}}
\newcommand{\gradG}{\cellcolor[HTML]{d1d8d6}}
\newcommand{\gradH}{\cellcolor[HTML]{f5f5f5}}
\newcommand{\gradI}{\cellcolor[HTML]{dfd6cf}}
\newcommand{\gradJ}{\cellcolor[HTML]{c8b8aa}}
\newcommand{\gradK}{\cellcolor[HTML]{b29a87}}
\newcommand{\gradL}{\cellcolor[HTML]{9b7e65}}
\newcommand{\gradM}{\cellcolor[HTML]{846344}\color{white}}
\newcommand{\gradN}{\cellcolor[HTML]{6c4925}\color{white}}
\newcommand{\gradO}{\cellcolor[HTML]{543005}\color{white}}


==> shading-gradations/Grays.tex <==
\newcommand{\gradA}{\cellcolor[HTML]{000000}\color{white}}
\newcommand{\gradB}{\cellcolor[HTML]{161616}\color{white}}
\newcommand{\gradC}{\cellcolor[HTML]{242424}\color{white}}
\newcommand{\gradD}{\cellcolor[HTML]{333333}\color{white}}
\newcommand{\gradE}{\cellcolor[HTML]{434343}\color{white}}
\newcommand{\gradF}{\cellcolor[HTML]{545454}\color{white}}
\newcommand{\gradG}{\cellcolor[HTML]{656565}\color{white}}
\newcommand{\gradH}{\cellcolor[HTML]{777777}\color{white}}
\newcommand{\gradI}{\cellcolor[HTML]{898989}}
\newcommand{\gradJ}{\cellcolor[HTML]{9c9c9c}}
\newcommand{\gradK}{\cellcolor[HTML]{afafaf}}
\newcommand{\gradL}{\cellcolor[HTML]{c2c2c2}}
\newcommand{\gradM}{\cellcolor[HTML]{d6d6d6}}
\newcommand{\gradN}{\cellcolor[HTML]{eaeaea}}
\newcommand{\gradO}{\cellcolor[HTML]{ffffff}}

==> shading-gradations/RedYellowGreen.tex <==
\newcommand{\gradA}{\cellcolor[HTML]{ee0c31}}
\newcommand{\gradB}{\cellcolor[HTML]{f74a28}}
\newcommand{\gradC}{\cellcolor[HTML]{fc6e20}}
\newcommand{\gradD}{\cellcolor[HTML]{ff8d1e}}
\newcommand{\gradE}{\cellcolor[HTML]{ffaa27}}
\newcommand{\gradF}{\cellcolor[HTML]{ffc639}}
\newcommand{\gradG}{\cellcolor[HTML]{fde051}}
\newcommand{\gradH}{\cellcolor[HTML]{fafa6e}}
\newcommand{\gradI}{\cellcolor[HTML]{eafb60}}
\newcommand{\gradJ}{\cellcolor[HTML]{d8fb52}}
\newcommand{\gradK}{\cellcolor[HTML]{c2fc46}}
\newcommand{\gradL}{\cellcolor[HTML]{aafd3c}}
\newcommand{\gradM}{\cellcolor[HTML]{8cfe35}}
\newcommand{\gradN}{\cellcolor[HTML]{64ff32}}
\newcommand{\gradO}{\cellcolor[HTML]{05ff34}}

==> tables/replication.tex <==
    \nprounddigits{2}
    \npdecimalsign{.}
    \setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setlength{\extrarowheight}{.75ex}
\resizebox{\textwidth}{!}{
    \begin{tabular}{l l >{\columncolor{lightgray!75!white}}n{2}{2} n{2}{2} >{\columncolor{lightgray!75!white}}n{2}{2} n{2}{2} >{\columncolor{lightgray!75!white}}n{2}{2} n{2}{2} >{\columncolor{lightgray!75!white}}n{2}{2} n{2}{2} >{\columncolor{lightgray!75!white}}n{2}{2} n{2}{2} >{\columncolor{lightgray!75!white}}n{2}{2} n{2}{2} >{\columncolor{lightgray!75!white}}n{2}{2} n{2}{2} >{\columncolor{lightgray!75!white}}n{2}{2}}
    \multirow{4}{*}{\rotatebox{90}{Using}} 
    & {{\rotatebox{90}{$\mathbf{i}_t$}}} & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \xmark & \cmark \\
    & {{\rotatebox{90}{$\mathbf{h}_t$}}} & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark \\
    & {{\rotatebox{90}{$\mathbf{f}_t$}}} & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark \\
    & {{\rotatebox{90}{$\mathbf{c}_t$}}} & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark \\
    \toprule
    
    \multirow{7}{*}{\rotatebox{90}{MLM \quad (cf. \Cref{tab:mlm-acc})}} & \multirow{5}{*}{\rotatebox{90}{lrn}} & 14.51466040951865 & 48.328796880585806 & 53.924389396395 & 9.239169423069273 & 49.715772696903776 & 53.66473197937012 & 13.184626400470734 & 55.45087456703186 & 48.09900607381548 & 53.96701097488403 & 55.58030435017177 & 49.08254402024405 & 54.05265263148716 & 55.79230189323425 & 55.52683557782855 \\
    & & 15.5377453991345 & 49.74250708307539 & 53.73721974236625  & 9.629424874271665  & 47.7885548557554  & 53.95616378102984 & 13.560531820569718  & 55.52993927683149  & 48.92094135284424 & 53.41828550611224  & 55.58224064963204  & 49.43208524159023 & 54.02902109282357  & 55.32878977911813 & 55.90544598443168 \\
    && 
    \\
    && 
    \\
    && 
    \\
    \cmidrule{3-17}
    & $\mu$ \\
    & $\sigma$ \\
    \midrule
    
     \multirow{7}{*}{\rotatebox{90}{SemCor \quad (cf. \Cref{tab:wsd-acc})}} & \multirow{5}{*}{\rotatebox{90}{Cls}} & 58.41511973529246 & 66.83865178621502 & 64.46077056811171 & 57.32151870338175 & 66.65358084235321 & 63.88312489484606 & 57.8262576411867 & 65.71140149178397 & 66.94520778419606 & 64.46077056811171 & 65.75626717514441 & 66.77135326117436 & 64.4495541472716 & 65.87964780438562 & 65.98620380236666 \\
    && 
    \\
    && 
    \\
    && 
    \\
    && 
    \\
    \cmidrule{3-17}
    & $\mu$ \\
    & $\sigma$ \\
    \midrule

    
       % \parbox[t]{0mm}{\mathbf{\mu}ltirow{2}{*}{\rotatebox{90}{KNN}}} 
            %&  dev & 54.24204966850208 & 64.07461512529498 & 61.99572985728734 & 55.1972131700191 & 64.27688504326329 & 62.40588830205641 & 55.42757613214968 & 62.75424204966851 & 64.3836386110799 & 62.12495786043376 & 62.88347005281493 & 64.33868974042027 & 62.05191594561187 & 63.70940555118553 & 63.63074502753119\\
\multirow{14}{*}{\rotatebox{90}{WNUT-16 \quad (cf. \Cref{tab:ner-f1})}} &
\multirow{5}{*}{\rotatebox{90}{base}} &
17.848750518242634 & 41.089007750646483 & 34.19621631464284 & 5.4750277610560394 & 21.127019018113108 & 35.54991841127489 & {\npboldmath} 16.13341143007513 & 36.750592420761824 & {\npboldmath} 40.838626202830824 & {\npboldmath} 36.88560549196929 & 38.193522182732087 & 39.699279917548563 & {\npboldmath} 37.220598055020665 & {\npboldmath} 39.00648567214642 & 37.68621932212761 \\ 
& & 
17.830853439583677  & {\npboldmath} 41.12996769788408 & {\npboldmath} 35.543025518636495 & 5.414754887802049 & {\npboldmath} 40.90145168910101  & 34.875266146279466 & 11.438637210456397 & 38.500991643082844  & 39.70628688060332  & 34.721070530725684 & {\npboldmath} 39.084568617753657  & 42.135316062332445  & 37.001227326911745 & 37.873957556197935  & 39.005484323913436  \\
&&
17.61779393364203 & 40.07757394736976  & 34.787294331987684 &  5.430779583879673 & 40.470378480780766  & 35.32472136292023 & 16.03102765613383 & {\npboldmath} 39.942635911563834 & 39.78395704263365 & 19.51798070545313 & 38.279411916828365 & 39.63596158641731 & 37.048876184505336  & 38.57809669077404 & 38.41331565801886 \\
&&
{\npboldmath} 18.111311700754482 & 40.054351442793856 & 34.96755366258074 &  {\npboldmath} 5.8115993193920745  & 39.73441268179479  & 35.25903090154169  & 15.82926041328383 & 38.15988813429601  & 40.735466757801797  & 35.92345766316215 & 38.77375534222827  & 39.981929271791067  & 34.961327916861223  & 38.01752284307368  & {\npboldmath} 39.39895203131293 \\
&&
06.177425718534705 & 40.576290660471803 & 34.19419231025689 &  5.352284934148882 & 40.524189740937133 & {\npboldmath} 36.07256882095743 & 15.708077947916302 & 38.306191255695277  & 40.44674169178297 & 34.19897307058529  & 37.709550867699293  & {\npboldmath} 42.30148622669703 & 35.41988005489388 & 15.277707305010185 & 38.56717882777792 \\
\cmidrule{3-17} 
& $\mu$ & 15.517227062151509 & 40.5854382998332 & 34.73765642762093 & 5.496889297255744 & 36.551490322145355 & 35.41630112859474 & 15.028082931573095 & 38.332059873079956 & 40.302215715130515 & 32.2494174923791 & 38.40816178544834 & 40.75079461295728 & 36.33038190763857 & 33.75075401344044 & 38.614230032630154 \\
& $\sigma$ & 4.67252424440406 & 0.4669384513322848 & 0.5084184646055521 & 0.16220191247120086 & 7.721495952500897 & 0.393543007092511 & 1.800891355658075 & 1.0152679167980838 & 0.4732977208179074 & 6.434160841913204 & 0.477888847677015 & 1.2050920188329255 & 0.9446771771377586 & 9.245382966487805 & 0.5783861713898768 \\ 
\cmidrule{2-17} 
 & \multirow{5}{*}{\rotatebox{90}{tune}} &
18.081620841351329 & 42.25024702479604 & 44.896204481295043 & 12.360316254946753 & 46.96394488986605 & 44.466470169295313 & 16.796041484809732 & 43.531872430370677 & 46.42991881347537 & 45.08474162787778 & 42.954413166002475 & 46.48613477794952 & {\npboldmath} 45.59531346054527 & {\npboldmath} 44.37682566405073 & 43.53840437464772 \\
&&
 6.0966800716939454 & 48.07495501371665  & 44.71908729335716  &  8.914195091006685  & {\npboldmath} 48.542410764668603 & {\npboldmath} 45.730790990932996 &  6.50080446175976  & 44.2254548408415  & 48.219669571102586  & 44.686457982777733 & 43.9828464093366  & 48.21302230117908 & 43.96093380200615 & 44.375536034134166  & 44.40652296177052
\\ &&
17.18347429819532 & {\npboldmath} 48.08654846162811 & {\npboldmath} 45.53955757401611  & 12.39985629818936 & 46.97272673505828  & 43.97191769576951 &  5.5058760522748704  & 43.337282446073716  & 49.295465364239 & 44.747321379292  & 44.83741631930682 & 47.32814927023877 & 44.609608486929736 & 44.054686656100417 & {\npboldmath} 44.52155571213461 
\\ &&
{\npboldmath} 18.24928198169917  & 45.52000920865189 & 44.797228347851714  &  5.248312292953712  & 46.07818901956332  & 44.93022905301821  & 16.539947703622787 & 43.419905555479854  & 47.72620490328259 & {\npboldmath} 45.29514109558921  & {\npboldmath} 44.9185223749056  & 46.46610464356285 & 44.8071036583237 & 43.69167584105111  & 43.872065565952323
\\ &&
13.207331194873914 & 46.72850868517987 & 45.31615251262241 & {\npboldmath} 12.778347947498514  & 47.287122603631476 & 44.51253551966562 & {\npboldmath} 17.725920797061911 & {\npboldmath} 44.65437348985219 & {\npboldmath} 50.57042122249079 & 44.900030422709547 & 44.173921836643376  & {\npboldmath} 48.636547151391873  & 44.166945875901825  & 44.021590586789083  & 43.458658781023746 
\\
\cmidrule{3-17} 
& $\mu$ & 14.563677677562737 & 46.132053678794506 & 45.053646041828486 & 10.340205576919004 & 47.16887880255754 & 44.72238868573633 & 12.613718099905812 & 43.83377775252359 & 48.448335974918066 & 44.94273850164925 & 44.17342402123897 & 47.42599162886442 & 44.62798105674134 & 44.104062956425096 & 43.959441479105784 \\
& $\sigma$ & 4.611998737265308 & 2.1630393135801818 & 0.3185865971028512 & 2.9061462311985964 & 0.7963227225586794 & 0.5886955363423204 & 5.420901326077246 & 0.5168622474106399 & 1.4048945474076526 & 0.22362647971313654 & 0.709699213426807 & 0.8830797250747199 & 0.5702034575815337 & 0.25589059002070047 & 0.43624405264563565\\ 
\bottomrule
    \end{tabular}}
